Enhancing Automotive User Experience with Dynamic Service Orchestration for Software Defined Vehicles

With the increasing demand for dynamic behaviors in automotive use cases, Software Defined Vehicles (SDVs) have emerged as a promising solution by bringing dynamic onboard service management capabilities. While users may request a wide range of services during vehicle operation, background tasks such as cooperative Vehicle-to-Everything (V2X) services can activate on-the-fly in response to real-time road conditions. In this dynamic environment, the efficient allocation of onboard resources becomes a complex challenge, in order to meet mixed-criticality onboard Quality-of-Service (QoS) network requirements while ensuring an optimal user experience. Additionally, the ever-evolving real-time network connectivity and computational availability conditions further complicate the process. In this context, we present a dynamic resource-based onboard service orchestration algorithm that considers real-time in-vehicle and V2X network health, along with onboard resource constraints, to select degraded modes for onboard applications and maximize user experience. To enable dynamic orchestration, we introduce the concept of Automotive eXperience Integrity Level (AXIL) which expresses a runtime priority for non-safety-critical applications. This algorithm produces near-optimal solutions while significantly reducing execution time compared to straightforward methods as demonstrated by simulation results. With this approach, we aim to enable efficient onboard execution for a user experience-focused service orchestration.

==> sections/07_guidelines.tex <==
\section{Engineering guidelines} \label{sec:engineering_guidelines}

In this section, we summarize the important parameters and considerations to have when deploying this solution in an industrial setting, along with future use cases and benefits.


\subsubsection{Scope}

Our proposed methodology is a runtime approach for orchestrating non-safety-critical onboard applications in a single vehicle. It is not designed for safety-critical applications, which could rather be pre-computed and pre-configured using our previous work \cite{laclauPredictive2023}. It is also not suited for a multi-vehicle environment, which would require a different approach to account for cooperative V2X use cases and edge computing with additional activation requirements.


\subsubsection{Assumptions}

In this work, we assume that all applications are already installed on the vehicle and available to be launched immediately. Each application developer defines a manifest with degraded modes and dependencies, and implements the onboard API provided by the infrastructure to switch execution modes when required by the orchestration engine. We also assume that all applications have a pre-assigned software context or ECU to be executed on, either fixed in the manifest or calculated at runtime by an orchestrator.


\subsubsection{Timing}

When implementing this approach, the following timing considerations must be taken into account. The algorithm does not provide any real-time response guarantees, and the execution time depends on the number of applications, modes, and resources. With the current state of this work, the cost of calling the algorithm may not be insignificant and should be considered when integrating it in the vehicle. Future strategies may optimize the selection of execution times based on resource availability dynamics to reduce the overall onboard overhead. Finally, due to the polynomial complexity of the current heuristic, the number of applications and resources should be kept as low as possible to ensure a fast response time. If the vehicle requires a response time guarantee $t$, it can use the best candidate at time $t$ as a temporary first approximation. The solutions for the most common requests could also be pre-computed offboard and stored in a lookup table, depending on the onboard storage capabilities.

Finally, while our approach is designed to be called on context or resource availability changes, future work could optimize the algorithm to predict future events and proactively switch to the best runtime modes at optimal times. Optionally, applications could also define \textit{greedy} modes where an application temporarily consumes more resources than necessary to cache more data. This can be useful if, for instance, the vehicle pre-fetches more data before entering a tunnel with poor network health. This last strategy can contribute to reduce the onboard overhead and improve the overall user experience.


\subsubsection{Implementation}

We assume that the global vehicle state is available to the infrastructure to obtain the current resource availabilities at all times. If this step fails, the vehicle may need to fall back to a pre-defined default behavior. As our solution autonomously optimizes user experience, this solution becomes extremely scalable for automakers. With many vehicle variants and heterogeneous physical E/E topologies, they do not need to manually generate state management policies.


\subsubsection{Configuration}

Our heuristic requires no configuration or calibration, but the values defined as the AXIL scores and resource requirements must be carefully selected to ensure a good user experience. The AXIL scores can either be defined by the application developers or the automaker based on user feedback, marketing strategies, or user preferences. Depending on user satisfaction and feedback, these scores can be progressively improved using existing strategies already deployed in other industries \cite{triki_learning_2017}. Resource requirements must be defined by the application developers and could be expressed in a technology-agnostic unit to avoid high software-hardware coupling. Optionally, additional constraints such as peripheral access or software context defined in the manifest would be used by the onboard scheduler to ensure the application is executed on the correct ECU and with the correct privileges.


\subsubsection{Additional settings}

While this work covers the main concept, several additional settings can be added to the algorithm to further improve flexibility. First, state management constraints can be easily added to the algorithm by setting a minimum and maximum mode to be selected for each application. This can be used to enforce a minimum user experience, which coincidentally improves solve speed. Second, the vehicle can select a subset of applications to be selected within the main matrix depending on the current context, as long as all dependencies can be met. Third, if the in-vehicle network has pre-allocated QoS slots currently available, they can be considered as additional resources to enable the most relevant application requiring it. Finally, the onboard architecture could consider the internal state of each application to decide when to reconfigure. This may be necessary if some applications enter temporary safety-critical states or to reduce disturbance.


\subsubsection{Benefits for the automotive industry}

This dynamic approach is a complete paradigm change for the automotive industry, currently used to regular OTA updates containing static components. While this new switch represents a difficult challenge, it has the potential of bringing new use cases and benefits for the users, manufacturers, and application developers. First, by consider mutual exclusive usage patterns as a foundational concept, dynamic architectures immediately benefit from using less hardware for the same amount of embedded features. This can either lower manufacturing costs and reduce the hardware environmental footprint, or provide more features for the same hardware. Second, it becomes easier to implement shared vehicles and a strong app ecosystem with personalized experiences based on the user preferences.

% \todo Add that background dependencies can have AXIL set to 0 for all modes, so that they are only enabled when needed. E.g. network proxy for a video streaming app.
